Beyond Grounding: Extracting Fine-Grained Event Hierarchies Across Modalities

Events describe happenings in our world that are of importance. Naturally, understanding events mentioned in multimedia content and how they are related forms an important way of comprehending our world. Existing literature can infer if events across textual and visual (video) domains are identical (via grounding) and thus, on the same semantic level. However, grounding fails to capture the intricate cross-event relations that exist due to the same events being referred to on many semantic levels. For example, in Figure 1, the abstract event of "war" manifests at a lower semantic level through subevents "tanks firing" (in video) and airplane "shot" (in text), leading to a hierarchical, multimodal relationship between the events. In this paper, we propose the task of extracting event hierarchies from multimodal (video and text) data to capture how the same event manifests itself in different modalities at different semantic levels. This reveals the structure of events and is critical to understanding them. To support research on this task, we introduce the Multimodal Hierarchical Events (MultiHiEve) dataset. Unlike prior video-language datasets, MultiHiEve is composed of news video-article pairs, which makes it rich in event hierarchies. We densely annotate a part of the dataset to construct the test benchmark. We show the limitations of state-of-the-art unimodal and multimodal baselines on this task. Further, we address these limitations via a new weakly supervised model, leveraging only unannotated video-article pairs from MultiHiEve. We perform a thorough evaluation of our proposed method which demonstrates improved performance on this task and highlight opportunities for future research.

==> tables/table-ab-feat-old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\caption{Ablation studies on features. ``CT'' denotes the contextual transformer. ``CS'' denotes the common-sense knowledge features. ``SF'' denotes the substraction of textural and visual features. ``MF'' denotes the element-wise product of textural and visual features.}
\label{tab:network-arch}
\begin{tabular}{c cccc rrr rrr r}
\toprule
 &    &    &    &    & \multicolumn{3}{c}{Hierarchical}                                       & \multicolumn{3}{c}{Identical}                                          &            \multirow{2}{*}{Avg F1}   \\
 \cmidrule(lr){6-8} \cmidrule(lr){9-11}
 & CT & CS & SF & MF & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \\
\toprule
 &    &    &    &    & 12.1                 & \textbf{30.7}        & 17.4                  & 7.2                  & 42.8                 & 12.4                  & 14.9                                            \\
 & \cmark  &    &    &    & 17.4                 & 23.9                 & 20.1                  & 7.5                  & 43.3                 & 12.8                  & 16.5                                            \\
 &    & \cmark  &    &    & 13.4                 & 29.1                 & 18.4                  & 7.6                  & 44.9                 & 13.0                  & 15.7                                            \\
 & \cmark  & \cmark  &    &    & 16.3                 & 22.4                 & 18.9                  & 7.2                  & 42.4                 & 12.4                  & 15.7                                            \\
 & \cmark  & \cmark  & \cmark  &    & 14.7                 & 29.9                 & 19.7                  & 7.6                  & 42.4                 & 12.8                  & 16.3                                            \\
 & \cmark  & \cmark  &    & \cmark  & 16.8                 & 24.9                 & 20.1                  & 7.7                  & \textbf{45.2}        & 13.2                  & 16.7                                            \\
 & \cmark  &  & \cmark  & \cmark  & 19.3 & 24.2                 & 21.5         & 7.6         & 44.3    & 13.0       & 17.3 \\                       
 & \cmark  & \cmark  & \cmark  & \cmark  & \textbf{21.9}        & 22.1                 & \textbf{22.0}         & \textbf{8.2}         & 44.5                 & \textbf{13.9}         & \textbf{18.0} \\                       
\bottomrule
\end{tabular}
\end{table}

==> tables/table-ab-feat.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\small

%``CT'': Contextual transformer. ``CS'': Common-sense Knowledge. ``EI'': Embedding Interactions.}
%including the subtraction and element-wise product of textural and visual features.}
% ``SF'' denotes the substraction of textural and visual features. ``MF'' denotes the element-wise product of textural and visual features.}

\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{l rrr rrr r}
\toprule
 & \multicolumn{3}{c}{Hierarchical}                                       & \multicolumn{3}{c}{Identical}                                          &            \multirow{2}{*}{Avg F1}   \\
 \cmidrule(lr){2-4} \cmidrule(lr){5-7}
 & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \\
\toprule
MASHER Basic & 12.1                 & \textbf{30.7}        & 17.4                  & 7.2                  & 42.8                 & 12.4                  & 14.9                                            \\
\quad + CT & 17.4                 & 23.9                 & 20.1                  & 7.5                  & 43.3                 & 12.8                  & 16.5                                            \\
\quad + CS & 13.4                 & 29.1                 & 18.4                  & 7.6                  & 44.9                 & 13.0                  & 15.7                                            \\
\quad + CT + CS + EI & \textbf{21.9}        & 22.1                 & \textbf{22.0}         & \textbf{8.2}         & 44.5                 & \textbf{13.9}         & \textbf{18.0} \\                       
\bottomrule
\end{tabular}
\caption{Ablation studies on components and features. ``MASHER Basic'': Basic MASHER model.}
\label{tab:network-arch}
\end{table}

==> tables/table-ab-focal.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\caption{Ablation studies on the hyperparameter of focal loss.}
\label{tab:focal-loss}
\begin{tabular}{l rrr rrr r}      
\toprule
& \multicolumn{3}{c}{Hierarchical}                                       & \multicolumn{3}{c}{Identical}                                          &                         \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7}                                        & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multirow{-2}{*}{Avg F1} \\
                                   
\toprule

$\lambda=1$               & 16.2                  & 23.4                  & 19.2                   & \textbf{7.8}                   & \textbf{42.8}                  & \textbf{13.2}                   & 16.2                                             \\
$\lambda=2$                   & \textbf{17.6}                  & 33.8                  & \textbf{23.1}                   & \textbf{7.8}                   & \textbf{42.8}                  & \textbf{13.2}                   & \textbf{18.2}                                            \\
$\lambda=5$ & 13.7                  & \textbf{34.5}                  & 19.6                   & \textbf{7.8}                   & 40.8                  & 13.1                   & 16.4   \\
\bottomrule
\end{tabular}
\end{table}

==> tables/table-dataset-comp-rebuttal.tex <==

\begin{table}[t]
\centering
\captionsetup{skip=3pt}
% \footnotesize
\fontsize{9}{11}\selectfont
% \setlength{\tabcolsep}{4pt}
\setlength{\tabcolsep}{3pt}
\scalebox{1.0}{
\begin{tabular}{lcccc}
\toprule
Dataset      & \#Vids. & \#Article Sents. & ASR & E2E Rels.  \\
\midrule
VidSitu~[{\color{green}{43}}]        & 29.2K   & -          & -                          & Visual                         \\
HowTo100M~[{\color{green}{31}}]         & 1.2M   & -          & \cmark                          & -                     \\
MERLOT~[{\color{green}{62}}] & 180M & - & \cmark & - \\
{\fontfamily{qcr}\selectfont MultiHiEve} & 100K   & \textbf{1.9M} & \cmark                          & \textbf{Multimodal}   \\
\bottomrule
\end{tabular}
}
\caption{Dataset Comparison. E2E Rels.: Event-Event Relations.}
\label{tab:rebuttal-dataset-comp}
\end{table}


==> tables/table-dataset-train.tex <==
\begin{table}[t]
\centering
\small
% \resizebox{!}{\textwidth}{
\setlength{\tabcolsep}{2pt}
% \scalebox{0.90}{
\begin{tabular}{l l llll l}
\toprule
Dataset       & Domain  & \#Vids & Avg. len. & \#Hrs. & ASR & \#Sent. \\
\midrule
MSVD~\cite{chen2011collecting}         & Open    & 1970                          & 10                                       & 5.3                                & No  & 70K                              \\
% MPII Cooking~\cite{rohrbach2012database}  & Cooking & 44                            & 600                                      & 8                                  & No  & 5609                             \\
% TACoS~\cite{regneri2013grounding}         & Cooking & 127                           & 360                                      & 15.9                               & No  & 18K                              \\
% TACos-MLevel~\cite{rohrbach2014coherent}  & Cooking & 185                           & 360                                      & 27.1                               & No  & 53K                              \\
% M-VAD~\cite{torabi2015using}         & Movie   & 92                            & 6.2                                      & 84.6                               & No  & 56K                              \\
MSR-VTT~\cite{xu2016msr}       & Open    & 7180                          & 20                                       & 41.2                               & No  & 200K                             \\
Charades~\cite{sigurdsson2016hollywood}      & Human   & 9848                          & 30                                       & 82.01                              & No  & 28K                              \\
% VTW~\cite{zeng2016generation}           & Open    & 18.1K                         & 90                                       & 213.2                              & No  & 45K                              \\
% YouCook II~\cite{ZhXuCoAAAI18}    & Cooking & 2000                          & 316                                      & 176                                & No  & 15K                              \\
ActyNet Cap~\cite{krishna2017dense}   & Open    & 20K                           & 180                                      & 849                                & No  & 100K                             \\
\midrule
{\fontfamily{qcr}\selectfont MultiHiEve} & News    & 100K                          & 148.9                                    & 4.1K %{4138.86}
& Yes & 1.9M    \\ 
\bottomrule
\end{tabular}
% }
\caption{Comparison of the training data of related video datasets. \#Vids: Number of Videos. Avg. sec.: Average length of videos in seconds. \#Hrs: Total number of video hours in the dataset. \#Sent.: Total number of sentences in the dataset.}
\label{tab:train-dataset}
\end{table}

==> tables/table-test.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering

\begin{tabular}{l rrr rrr r}
\toprule
                                        & \multicolumn{3}{c}{Hierarchical}                                       & \multicolumn{3}{c}{Identical}                                          &   \multirow{2}{*}{Avg F1}                       \\
                     \cmidrule(lr){2-4} \cmidrule(lr){5-7}   
                                        & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} &  \\ 
\toprule
Prior Baseline                   & 2.0                  & 2.0                  & 2.0                    & 1.2                  & 1.2                  & 1.2                    & 1.6                                            \\
Text Only Baseline               &   2.1     &  0.1      &          0.1     &   2.6    &  13.6   &  4.3  & 2.2                           \\
Multimodal Baseline & \textbf{28.0}     & 6.3                 & 10.3           & \textbf{7.6}             & 32.3                 & \textbf{12.4}      & 11.4                                            \\ \hline
MERP                                    & 11.9        & \textbf{18.8}        & \textbf{14.6}          & 6.3         & \textbf{39.0}        & 10.9          & \textbf{12.8}  \\     
\bottomrule
\end{tabular}
\caption{Comparison with baseline models on the test set.}
\label{tab:baselines-test}
\end{table}

==> tables/table-val.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\caption{Comparison with baseline models on the validation set.}
\label{tab:baselines-val}
\begin{tabular}{l rrr rrr r}
\toprule
                                        & \multicolumn{3}{c}{Hierarchical}                                       & \multicolumn{3}{c}{Identical}                                          &   \multirow{2}{*}{Avg F1}                       \\
                     \cmidrule(lr){2-4} \cmidrule(lr){5-7}   
                                        & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} &  \\ 
\toprule
Prior Baseline                   & 4.7                  & 4.7                  & 4.7                    & 2.0                  & 2.0                  & 2.0                    & 3.4                                             \\
Text Only Baseline               & 5.9                  & 0.1                  & 0.1                    & 2.5                  & 7.1                  & 3.6                    & 1.9                                             \\
Multimodal Baseline & \textbf{35.7}                 & 5.0                  & 8.8                    & \textbf{8.8}                  & 33.1                 & \textbf{13.9}                   & 11.4                                            \\ \hline
MERP &   21.9 &	\bf 22.1 &	\bf 22.0 &	8.2	& \bf 44.5	& \bf 13.9	& \bf 18.0  \\   
\bottomrule
\end{tabular}
\end{table}
